Fashion-VDM: Video Diffusion Model for Virtual Try-On

We present Fashion-VDM, a video diffusion model (VDM) for generating virtual try-on videos. Given an input garment image and person video, our method aims to generate a high-quality try-on video of the person wearing the given garment, while preserving the person's identity and motion. Image-based virtual try-on has shown impressive results; however, existing video virtual try-on (VVT) methods are still lacking garment details and temporal consistency. To address these issues, we propose a diffusion-based architecture for video virtual try-on, split classifier-free guidance for increased control over the conditioning inputs, and a progressive temporal training strategy for single-pass 64-frame, 512px video generation. We also demonstrate the effectiveness of joint image-video training for video try-on, especially when video data is limited. Our qualitative and quantitative experiments show that our approach sets the new state-of-the-art for video virtual try-on. For additional results, visit our project page: https://johannakarras.github.io/Fashion-VDM.

==> Sections/Ablations.tex <==
\section{Ablation Studies}\label{sec:ablations}
    %\input{Figures_Latex/joint-training}
 
    
    We ablate each of our design choices with respect to garment fidelity, temporal smoothness, and photorealism.
    We report quantitative results for each ablated version in Table~\ref{tab:ablations}. All components are essential to improving realism (FID), temporal consistency (FVD), and garment fidelity (CLIP). Qualitatively, we find that split-CFG and joint training have the largest effect on person/garment fidelity and overall quality (Figure \ref{fig:garment-fidelity}), while progressive training and temporal blocks affect the temporal smoothness (Figure \ref{fig:temporal-smoothness}). We discuss these effects in detail in the remainder of this section.
    
    \subsection{Split Classifier-Free Guidance}

    Split-CFG improves per-frame person and garment fidelity, thereby improving overall inter-frame temporal consistency and photrealism. In Figure \ref{fig:split-cfg-1}, we compare results generated with different split-CFG weights at inference time. By increasing the person guidance weight $w_p$ from 0 to 1, the realism and identity of the input person are improved. Increasing the full-conditional weight $w_\text{full}$ improves the garment fidelity, but not as much as by increasing the garment weight $w_g$ alone, as in the last column. We provide quantitative split-CFG ablation results in the Supplementary. In the Supplementary, we demonstrate that increasing $w_g$ also increases fine-grain garment details when using a version of our model trained on limited video data. This suggests split-CFG does not require extensive training to be useful and can be impactful in low-resource settings.

    \subsection{Joint Image-Video Training}

    We find that training with video data only in the temporal phases sacrifices garment fidelity compared to the base image model. %, due to the limited size of the video dataset in comparison to the image dataset. 
    Training jointly with images and videos increases the fidelity to garment details, even compared to the image baseline, as shown by the improved FID and CLIP scores in Table~\ref{tab:ablations}. The increased access to diverse data with joint image-video training also enables the model to synthesize more plausible occluded regions. For example, as shown in Figure \ref{fig:joint-training}, the jointly trained model is able to generate a hood with more realism than the video-only model.
    
    %This suggests that training jointly with images and videos benefits both image-based and video-based try-on models, and is a promising direction for future image try-on work.

    \subsection{Temporal Blocks}

    As seen in prior works~\cite{vdm, imagen-video}, interleaving 3D-convolution and temporal attention blocks into the 2D UNet greatly improves temporal consistency. Removing temporal blocks entirely causes large temporal inconsistencies. For instance, in the top row of Figure~\ref{fig:temporal-smoothness}, the ablated model without temporal blocks swaps the pants and body shape in each frame.

    \subsection{Progressive Temporal Training}
    \label{ssec:ablation-prog-training}

    To ablate our progressive training scheme, we train our image base model directly with 16-frame video batches for the same total number of iterations, but skipping the 8-frame training phase entirely. Progressive training enables more temporally smooth results with the same number of training iterations. This is supported by our quantitative findings in Table~\ref{tab:ablations}, which indicates worse FVD when not doing progressive training. Qualitatively, in Figure~\ref{fig:temporal-smoothness}, the non-progressively trained model in the middle row exhibits temporal artifacts in the pants region and intermittently merges the pant legs into a skirt. We hypothesize that, given limited training iterations, it is easier to learn temporal consistency well across a small number of frames. Then, to transfer that knowledge to larger temporal windows only requires minimal additional training. 
      
